CT-CLIP Representations for Multimodal Lung Cancer Survival Prediction

Accurate prognosis prediction is important for treatment planning in lung cancer, but deep learning-driven survival modelling is often limited by the scarcity of curated imaging cohorts with reliable outcome data. This study evaluates whether representations from a domain-specific foundation model can be used for multimodal survival prediction in data-constrained clinical settings. We assess the foundation model CT-CLIP as a feature extractor for pretreatment computed tomography images and clinical variables from 242 diagnosed lung cancer patients. The evaluation includes adaptation strategies based on frozen encoders, full fine-tuning, and low-rank adaptation, together with modality ablations and comparisons with clinical and multimodal baselines. The results show that a frozen CT-CLIP model combined with a trainable lightweight survival head outperforms the clinical baseline and achieves comparable or improved performance relative to other multimodal approaches, and separates patients into clinically meaningful high- and low-risk groups.

==> clip.tex <==
% This file was created with matplot2tikz v0.5.3.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
width=0.51\textwidth,
height=5.5cm,
x grid style={darkgray176},
xlabel={$t$ (days)},
xmin=-243.4, xmax=5111.4,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.0469616662841643, ymax=1.0498553174421,
tick style={draw=none},  % Removes the tick marks
ymajorticks=false,     % Optional: Alternative to remove y-tick labels
% ytick style={color=black}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.25]
(axis cs:0,1)
--(axis cs:0,1)
--(axis cs:198,1)
--(axis cs:198,0.748385024194756)
--(axis cs:301,0.748385024194756)
--(axis cs:301,0.716390337258063)
--(axis cs:594,0.716390337258063)
--(axis cs:594,0.672561452863359)
--(axis cs:775,0.672561452863359)
--(axis cs:775,0.628056081556178)
--(axis cs:853,0.628056081556178)
--(axis cs:853,0.584449088202953)
--(axis cs:1232,0.584449088202953)
--(axis cs:1232,0.542048122466753)
--(axis cs:1281,0.542048122466753)
--(axis cs:1281,0.50088720143207)
--(axis cs:1303,0.50088720143207)
--(axis cs:1303,0.460934451282713)
--(axis cs:1628,0.460934451282713)
--(axis cs:1628,0.42214773839249)
--(axis cs:1687,0.42214773839249)
--(axis cs:1687,0.384491392675349)
--(axis cs:2135,0.384491392675349)
--(axis cs:2135,0.384491392675349)
--(axis cs:2233,0.384491392675349)
--(axis cs:2233,0.344112745147404)
--(axis cs:2288,0.344112745147404)
--(axis cs:2288,0.344112745147404)
--(axis cs:2390,0.344112745147404)
--(axis cs:2390,0.344112745147404)
--(axis cs:2827,0.344112745147404)
--(axis cs:2827,0.294852755834642)
--(axis cs:2838,0.294852755834642)
--(axis cs:2838,0.294852755834642)
--(axis cs:2958,0.294852755834642)
--(axis cs:2958,0.241558286230582)
--(axis cs:3024,0.241558286230582)
--(axis cs:3024,0.241558286230582)
--(axis cs:3152,0.241558286230582)
--(axis cs:3152,0.241558286230582)
--(axis cs:3762,0.241558286230582)
--(axis cs:3762,0.241558286230582)
--(axis cs:3802,0.241558286230582)
--(axis cs:3802,0.241558286230582)
--(axis cs:4220,0.241558286230582)
--(axis cs:4220,0.11937478242737)
--(axis cs:4615,0.11937478242737)
--(axis cs:4615,0.11937478242737)
--(axis cs:4775,0.11937478242737)
--(axis cs:4775,0.0137001250535222)
--(axis cs:4868,0.0137001250535222)
--(axis cs:4868,0.0137001250535222)
--(axis cs:4868,0.478286393528511)
--(axis cs:4868,0.478286393528511)
--(axis cs:4868,0.478286393528511)
--(axis cs:4775,0.478286393528511)
--(axis cs:4775,0.574310441297567)
--(axis cs:4615,0.574310441297567)
--(axis cs:4615,0.574310441297567)
--(axis cs:4220,0.574310441297567)
--(axis cs:4220,0.63872568882974)
--(axis cs:3802,0.63872568882974)
--(axis cs:3802,0.63872568882974)
--(axis cs:3762,0.63872568882974)
--(axis cs:3762,0.63872568882974)
--(axis cs:3152,0.63872568882974)
--(axis cs:3152,0.63872568882974)
--(axis cs:3024,0.63872568882974)
--(axis cs:3024,0.63872568882974)
--(axis cs:2958,0.63872568882974)
--(axis cs:2958,0.684620285674525)
--(axis cs:2838,0.684620285674525)
--(axis cs:2838,0.684620285674525)
--(axis cs:2827,0.684620285674525)
--(axis cs:2827,0.725621140787015)
--(axis cs:2390,0.725621140787015)
--(axis cs:2390,0.725621140787015)
--(axis cs:2288,0.725621140787015)
--(axis cs:2288,0.725621140787015)
--(axis cs:2233,0.725621140787015)
--(axis cs:2233,0.761092652475561)
--(axis cs:2135,0.761092652475561)
--(axis cs:2135,0.761092652475561)
--(axis cs:1687,0.761092652475561)
--(axis cs:1687,0.793778313712923)
--(axis cs:1628,0.793778313712923)
--(axis cs:1628,0.825273134683081)
--(axis cs:1303,0.825273134683081)
--(axis cs:1303,0.85548429738792)
--(axis cs:1281,0.85548429738792)
--(axis cs:1281,0.884277637841535)
--(axis cs:1232,0.884277637841535)
--(axis cs:1232,0.911458059564583)
--(axis cs:853,0.911458059564583)
--(axis cs:853,0.93673324025134)
--(axis cs:775,0.93673324025134)
--(axis cs:775,0.959639832332033)
--(axis cs:594,0.959639832332033)
--(axis cs:594,0.97937058542805)
--(axis cs:301,0.97937058542805)
--(axis cs:301,0.994266950748838)
--(axis cs:198,0.994266950748838)
--(axis cs:198,1)
--(axis cs:0,1)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.25]
(axis cs:0,1)
--(axis cs:0,1)
--(axis cs:7,1)
--(axis cs:7,0.748385024194756)
--(axis cs:32,0.748385024194756)
--(axis cs:32,0.716390337258063)
--(axis cs:37,0.716390337258063)
--(axis cs:37,0.672561452863359)
--(axis cs:42,0.672561452863359)
--(axis cs:42,0.628056081556178)
--(axis cs:66,0.628056081556178)
--(axis cs:66,0.584449088202953)
--(axis cs:85,0.584449088202953)
--(axis cs:85,0.542048122466753)
--(axis cs:100,0.542048122466753)
--(axis cs:100,0.50088720143207)
--(axis cs:159,0.50088720143207)
--(axis cs:159,0.460934451282713)
--(axis cs:167,0.460934451282713)
--(axis cs:167,0.42214773839249)
--(axis cs:171,0.42214773839249)
--(axis cs:171,0.384491392675349)
--(axis cs:243,0.384491392675349)
--(axis cs:243,0.347941431122686)
--(axis cs:269,0.347941431122686)
--(axis cs:269,0.312487280636999)
--(axis cs:310,0.312487280636999)
--(axis cs:310,0.278132674620154)
--(axis cs:320,0.278132674620154)
--(axis cs:320,0.244896765738911)
--(axis cs:363,0.244896765738911)
--(axis cs:363,0.212816006017847)
--(axis cs:411,0.212816006017847)
--(axis cs:411,0.181947285130073)
--(axis cs:612,0.181947285130073)
--(axis cs:612,0.152373006149173)
--(axis cs:648,0.152373006149173)
--(axis cs:648,0.124209246821289)
--(axis cs:692,0.124209246821289)
--(axis cs:692,0.0976191295349579)
--(axis cs:774,0.0976191295349579)
--(axis cs:774,0.072835615144402)
--(axis cs:779,0.072835615144402)
--(axis cs:779,0.0502027986883727)
--(axis cs:964,0.0502027986883727)
--(axis cs:964,0.0302573652962818)
--(axis cs:1178,0.0302573652962818)
--(axis cs:1178,0.013908842770298)
--(axis cs:2532,0.013908842770298)
--(axis cs:2532,0.00289365115793875)
--(axis cs:4432,0.00289365115793875)
--(axis cs:4432,0.00289365115793875)
--(axis cs:4432,0.169893724196389)
--(axis cs:4432,0.169893724196389)
--(axis cs:4432,0.169893724196389)
--(axis cs:2532,0.169893724196389)
--(axis cs:2532,0.224887570799936)
--(axis cs:1178,0.224887570799936)
--(axis cs:1178,0.276605715875034)
--(axis cs:964,0.276605715875034)
--(axis cs:964,0.325444556902778)
--(axis cs:779,0.325444556902778)
--(axis cs:779,0.372011612693522)
--(axis cs:774,0.372011612693522)
--(axis cs:774,0.416716112310943)
--(axis cs:692,0.416716112310943)
--(axis cs:692,0.459830778869253)
--(axis cs:648,0.459830778869253)
--(axis cs:648,0.501541924891068)
--(axis cs:612,0.501541924891068)
--(axis cs:612,0.541978976429534)
--(axis cs:411,0.541978976429534)
--(axis cs:411,0.581231728746506)
--(axis cs:363,0.581231728746506)
--(axis cs:363,0.619360620067105)
--(axis cs:320,0.619360620067105)
--(axis cs:320,0.656402853600177)
--(axis cs:310,0.656402853600177)
--(axis cs:310,0.692375854684631)
--(axis cs:269,0.692375854684631)
--(axis cs:269,0.727278817455721)
--(axis cs:243,0.727278817455721)
--(axis cs:243,0.761092652475561)
--(axis cs:171,0.761092652475561)
--(axis cs:171,0.793778313712923)
--(axis cs:167,0.793778313712923)
--(axis cs:167,0.825273134683081)
--(axis cs:159,0.825273134683081)
--(axis cs:159,0.85548429738792)
--(axis cs:100,0.85548429738792)
--(axis cs:100,0.884277637841535)
--(axis cs:85,0.884277637841535)
--(axis cs:85,0.911458059564583)
--(axis cs:66,0.911458059564583)
--(axis cs:66,0.93673324025134)
--(axis cs:42,0.93673324025134)
--(axis cs:42,0.959639832332033)
--(axis cs:37,0.959639832332033)
--(axis cs:37,0.97937058542805)
--(axis cs:32,0.97937058542805)
--(axis cs:32,0.994266950748838)
--(axis cs:7,0.994266950748838)
--(axis cs:7,1)
--(axis cs:0,1)
--cycle;

\addplot [semithick, steelblue31119180, mark=+, mark size=6, mark options={solid}, only marks, forget plot]
table {%
2135 0.6
2288 0.557142857142857
2390 0.557142857142857
2838 0.506493506493507
3024 0.45021645021645
3152 0.45021645021645
3762 0.45021645021645
3802 0.45021645021645
4615 0.337662337662338
4868 0.168831168831169
};
\addplot [semithick, steelblue31119180, const plot mark left]
table {%
0 1
198 0.96
301 0.92
594 0.88
775 0.84
853 0.8
1232 0.76
1281 0.72
1303 0.68
1628 0.64
1687 0.6
2135 0.6
2233 0.557142857142857
2288 0.557142857142857
2390 0.557142857142857
2827 0.506493506493507
2838 0.506493506493507
2958 0.45021645021645
3024 0.45021645021645
3152 0.45021645021645
3762 0.45021645021645
3802 0.45021645021645
4220 0.337662337662338
4615 0.337662337662338
4775 0.168831168831169
4868 0.168831168831169
};
\addlegendentry{Low risk (CT-CLIP)}
\addplot [semithick, darkorange25512714, mark=+, mark size=6, mark options={solid}, only marks, forget plot]
table {%
4432 0.04
};
\addplot [semithick, darkorange25512714, const plot mark left]
table {%
0 1
7 0.96
32 0.92
37 0.88
42 0.84
66 0.8
85 0.76
100 0.72
159 0.68
167 0.64
171 0.6
243 0.56
269 0.52
310 0.48
320 0.44
363 0.4
411 0.36
612 0.32
648 0.28
692 0.24
774 0.2
779 0.16
964 0.12
1178 0.08
2532 0.04
4432 0.04
};
\addlegendentry{High risk (CT-CLIP)}

\draw[<->, semithick] (axis cs: 2000, 0.1) -- node[midway, left, font=\scriptsize, yshift=-33pt] {$p=0.000$} (axis cs: 2000, 0.59);
\end{axis}

\end{tikzpicture}


==> cox.tex <==
% This file was created with matplot2tikz v0.5.3.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
width=0.51\textwidth,
height=5.5cm,
x grid style={darkgray176},
xlabel={$t$ (days)},
ylabel={Survival probability},
xmin=-243.4, xmax=5111.4,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.05, ymax=1.05,
ytick style={color=black}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.25]
(axis cs:0,1)
--(axis cs:0,1)
--(axis cs:198,1)
--(axis cs:198,0.748385024194756)
--(axis cs:269,0.748385024194756)
--(axis cs:269,0.716390337258063)
--(axis cs:310,0.716390337258063)
--(axis cs:310,0.672561452863359)
--(axis cs:411,0.672561452863359)
--(axis cs:411,0.628056081556178)
--(axis cs:774,0.628056081556178)
--(axis cs:774,0.584449088202953)
--(axis cs:775,0.584449088202953)
--(axis cs:775,0.542048122466753)
--(axis cs:779,0.542048122466753)
--(axis cs:779,0.50088720143207)
--(axis cs:853,0.50088720143207)
--(axis cs:853,0.460934451282713)
--(axis cs:1232,0.460934451282713)
--(axis cs:1232,0.42214773839249)
--(axis cs:1281,0.42214773839249)
--(axis cs:1281,0.384491392675349)
--(axis cs:1303,0.384491392675349)
--(axis cs:1303,0.347941431122686)
--(axis cs:1687,0.347941431122686)
--(axis cs:1687,0.312487280636999)
--(axis cs:2135,0.312487280636999)
--(axis cs:2135,0.312487280636999)
--(axis cs:2233,0.312487280636999)
--(axis cs:2233,0.274018811002908)
--(axis cs:2288,0.274018811002908)
--(axis cs:2288,0.274018811002908)
--(axis cs:2390,0.274018811002908)
--(axis cs:2390,0.274018811002908)
--(axis cs:2827,0.274018811002908)
--(axis cs:2827,0.225229311160784)
--(axis cs:2838,0.225229311160784)
--(axis cs:2838,0.225229311160784)
--(axis cs:2958,0.225229311160784)
--(axis cs:2958,0.171361851386913)
--(axis cs:3024,0.171361851386913)
--(axis cs:3024,0.171361851386913)
--(axis cs:3152,0.171361851386913)
--(axis cs:3152,0.171361851386913)
--(axis cs:3802,0.171361851386913)
--(axis cs:3802,0.171361851386913)
--(axis cs:4220,0.171361851386913)
--(axis cs:4220,0.059251332844783)
--(axis cs:4615,0.059251332844783)
--(axis cs:4615,0.059251332844783)
--(axis cs:4868,0.059251332844783)
--(axis cs:4868,0.059251332844783)
--(axis cs:4868,0.490733014671999)
--(axis cs:4868,0.490733014671999)
--(axis cs:4868,0.490733014671999)
--(axis cs:4615,0.490733014671999)
--(axis cs:4615,0.490733014671999)
--(axis cs:4220,0.490733014671999)
--(axis cs:4220,0.559009815260044)
--(axis cs:3802,0.559009815260044)
--(axis cs:3802,0.559009815260044)
--(axis cs:3152,0.559009815260044)
--(axis cs:3152,0.559009815260044)
--(axis cs:3024,0.559009815260044)
--(axis cs:3024,0.559009815260044)
--(axis cs:2958,0.559009815260044)
--(axis cs:2958,0.609760430964132)
--(axis cs:2838,0.609760430964132)
--(axis cs:2838,0.609760430964132)
--(axis cs:2827,0.609760430964132)
--(axis cs:2827,0.654375315432333)
--(axis cs:2390,0.654375315432333)
--(axis cs:2390,0.654375315432333)
--(axis cs:2288,0.654375315432333)
--(axis cs:2288,0.654375315432333)
--(axis cs:2233,0.654375315432333)
--(axis cs:2233,0.692375854684631)
--(axis cs:2135,0.692375854684631)
--(axis cs:2135,0.692375854684631)
--(axis cs:1687,0.692375854684631)
--(axis cs:1687,0.727278817455721)
--(axis cs:1303,0.727278817455721)
--(axis cs:1303,0.761092652475561)
--(axis cs:1281,0.761092652475561)
--(axis cs:1281,0.793778313712923)
--(axis cs:1232,0.793778313712923)
--(axis cs:1232,0.825273134683081)
--(axis cs:853,0.825273134683081)
--(axis cs:853,0.85548429738792)
--(axis cs:779,0.85548429738792)
--(axis cs:779,0.884277637841535)
--(axis cs:775,0.884277637841535)
--(axis cs:775,0.911458059564583)
--(axis cs:774,0.911458059564583)
--(axis cs:774,0.93673324025134)
--(axis cs:411,0.93673324025134)
--(axis cs:411,0.959639832332033)
--(axis cs:310,0.959639832332033)
--(axis cs:310,0.97937058542805)
--(axis cs:269,0.97937058542805)
--(axis cs:269,0.994266950748838)
--(axis cs:198,0.994266950748838)
--(axis cs:198,1)
--(axis cs:0,1)
--cycle;

\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.25]
(axis cs:0,1)
--(axis cs:0,1)
--(axis cs:7,1)
--(axis cs:7,0.748385024194756)
--(axis cs:32,0.748385024194756)
--(axis cs:32,0.716390337258063)
--(axis cs:37,0.716390337258063)
--(axis cs:37,0.672561452863359)
--(axis cs:42,0.672561452863359)
--(axis cs:42,0.628056081556178)
--(axis cs:66,0.628056081556178)
--(axis cs:66,0.584449088202953)
--(axis cs:85,0.584449088202953)
--(axis cs:85,0.542048122466753)
--(axis cs:100,0.542048122466753)
--(axis cs:100,0.50088720143207)
--(axis cs:159,0.50088720143207)
--(axis cs:159,0.460934451282713)
--(axis cs:167,0.460934451282713)
--(axis cs:167,0.42214773839249)
--(axis cs:171,0.42214773839249)
--(axis cs:171,0.384491392675349)
--(axis cs:243,0.384491392675349)
--(axis cs:243,0.347941431122686)
--(axis cs:301,0.347941431122686)
--(axis cs:301,0.312487280636999)
--(axis cs:320,0.312487280636999)
--(axis cs:320,0.278132674620154)
--(axis cs:363,0.278132674620154)
--(axis cs:363,0.244896765738911)
--(axis cs:594,0.244896765738911)
--(axis cs:594,0.212816006017847)
--(axis cs:612,0.212816006017847)
--(axis cs:612,0.181947285130073)
--(axis cs:648,0.181947285130073)
--(axis cs:648,0.152373006149173)
--(axis cs:692,0.152373006149173)
--(axis cs:692,0.124209246821289)
--(axis cs:964,0.124209246821289)
--(axis cs:964,0.0976191295349579)
--(axis cs:1178,0.0976191295349579)
--(axis cs:1178,0.072835615144402)
--(axis cs:1628,0.072835615144402)
--(axis cs:1628,0.0502027986883727)
--(axis cs:2532,0.0502027986883727)
--(axis cs:2532,0.0302573652962818)
--(axis cs:3762,0.0302573652962818)
--(axis cs:3762,0.0302573652962818)
--(axis cs:4432,0.0302573652962818)
--(axis cs:4432,0.0302573652962818)
--(axis cs:4775,0.0302573652962818)
--(axis cs:4775,0)
--(axis cs:4775,0)
--(axis cs:4775,0)
--(axis cs:4775,0.276605715875034)
--(axis cs:4432,0.276605715875034)
--(axis cs:4432,0.276605715875034)
--(axis cs:3762,0.276605715875034)
--(axis cs:3762,0.276605715875034)
--(axis cs:2532,0.276605715875034)
--(axis cs:2532,0.325444556902778)
--(axis cs:1628,0.325444556902778)
--(axis cs:1628,0.372011612693522)
--(axis cs:1178,0.372011612693522)
--(axis cs:1178,0.416716112310943)
--(axis cs:964,0.416716112310943)
--(axis cs:964,0.459830778869253)
--(axis cs:692,0.459830778869253)
--(axis cs:692,0.501541924891068)
--(axis cs:648,0.501541924891068)
--(axis cs:648,0.541978976429534)
--(axis cs:612,0.541978976429534)
--(axis cs:612,0.581231728746506)
--(axis cs:594,0.581231728746506)
--(axis cs:594,0.619360620067105)
--(axis cs:363,0.619360620067105)
--(axis cs:363,0.656402853600177)
--(axis cs:320,0.656402853600177)
--(axis cs:320,0.692375854684631)
--(axis cs:301,0.692375854684631)
--(axis cs:301,0.727278817455721)
--(axis cs:243,0.727278817455721)
--(axis cs:243,0.761092652475561)
--(axis cs:171,0.761092652475561)
--(axis cs:171,0.793778313712923)
--(axis cs:167,0.793778313712923)
--(axis cs:167,0.825273134683081)
--(axis cs:159,0.825273134683081)
--(axis cs:159,0.85548429738792)
--(axis cs:100,0.85548429738792)
--(axis cs:100,0.884277637841535)
--(axis cs:85,0.884277637841535)
--(axis cs:85,0.911458059564583)
--(axis cs:66,0.911458059564583)
--(axis cs:66,0.93673324025134)
--(axis cs:42,0.93673324025134)
--(axis cs:42,0.959639832332033)
--(axis cs:37,0.959639832332033)
--(axis cs:37,0.97937058542805)
--(axis cs:32,0.97937058542805)
--(axis cs:32,0.994266950748838)
--(axis cs:7,0.994266950748838)
--(axis cs:7,1)
--(axis cs:0,1)
--cycle;

\addplot [semithick, steelblue31119180, mark=+, mark size=6, mark options={solid}, only marks, forget plot]
table {%
2135 0.52
2288 0.476666666666667
2390 0.476666666666667
2838 0.423703703703704
3024 0.363174603174603
3152 0.363174603174603
3802 0.363174603174603
4615 0.242116402116402
4868 0.242116402116402
};
\addplot [semithick, steelblue31119180, const plot mark left]
table {%
0 1
198 0.96
269 0.92
310 0.88
411 0.84
774 0.8
775 0.76
779 0.72
853 0.68
1232 0.64
1281 0.6
1303 0.56
1687 0.52
2135 0.52
2233 0.476666666666667
2288 0.476666666666667
2390 0.476666666666667
2827 0.423703703703704
2838 0.423703703703704
2958 0.363174603174603
3024 0.363174603174603
3152 0.363174603174603
3802 0.363174603174603
4220 0.242116402116402
4615 0.242116402116402
4868 0.242116402116402
};
\addlegendentry{Low risk (Cox)}
\addplot [semithick, darkorange25512714, mark=+, mark size=6, mark options={solid}, only marks, forget plot]
table {%
3762 0.12
4432 0.12
};
\addplot [semithick, darkorange25512714, const plot mark left]
table {%
0 1
7 0.96
32 0.92
37 0.88
42 0.84
66 0.8
85 0.76
100 0.72
159 0.68
167 0.64
171 0.6
243 0.56
301 0.52
320 0.48
363 0.44
594 0.4
612 0.36
648 0.32
692 0.28
964 0.24
1178 0.2
1628 0.16
2532 0.12
3762 0.12
4432 0.12
4775 0
};
\addlegendentry{High risk (Cox)}

\draw[<->, semithick] (axis cs: 2000, 0.18) -- node[midway, left, font=\scriptsize, yshift=-25pt] {$p=0.001$} (axis cs: 2000, 0.51);
\end{axis}




\end{tikzpicture}


==> cube.tex <==
\begin{tikzpicture}[scale=2,
    x={(1cm,0cm)},
    y={(0.5cm,0.5cm)},
    z={(0cm,1cm)}
]

% Define cube vertices
\coordinate (A) at (0,0,0);
\coordinate (B) at (1,0,0);
\coordinate (C) at (1,0.7,0);
\coordinate (D) at (0,0.7,0);

\coordinate (E) at (0,0,1);
\coordinate (F) at (1,0,1);
\coordinate (G) at (1,0.7,1);
\coordinate (H) at (0,0.7,1);

% Draw back face
\filldraw[fill=black!100, draw=gray] (E) -- (F) -- (G) -- (H) -- cycle;

% Draw bottom face
\filldraw[fill=black!100, draw=gray] (A) -- (B) -- (F) -- (E) -- cycle;

% Draw side face
\filldraw[fill=black!100, draw=gray] (B) -- (C) -- (G) -- (F) -- cycle;

% Draw front edges
\draw[black] (A) -- (B) -- (C) -- (D) -- cycle;
\draw[black] (A) -- (E);
\draw[black] (D) -- (H);
\draw[black] (C) -- (G);

\end{tikzpicture}
